Quantum Correlations in Space-Time: Foundations and Applications

The absolute/relative debate on the nature of space and time is ongoing for thousands of years. Here we attempt to investigate space and time from the information theoretic point of view to understand spatial and temporal correlations under the relative assumption. Correlations, as a measure of relationship between two quantities, do not distinguish space and time in classical probability theory; quantum correlations in space are well-studied but temporal correlations are not well understood. The thesis investigates quantum correlations in space-time, by treating temporal correlations equally in form as spatial correlations and unifying quantum correlations in space and time. In particular, we follow the pseudo-density matrix formalism in which quantum states in spacetime are properly defined by correlations from measurements. We first review classical correlations, quantum correlations in space and time, to motivate the pseudo-density matrix formalism in finite dimensions. Next we generalise the pseudo-density matrix formulation to the Gaussian case, general continuous variables via Wigner representations, and general measurement processes like weak measurements. Then we compare the pseudo-density matrix formalism with other spacetime formulations: indefinite causal structures, consistent histories, generalised non-local games, out-of-time-order correlation functions, and path integrals. We argue that in non-relativistic quantum mechanics, different spacetime formulations are closely related via quantum correlations, except path integrals. Finally, we apply the pseudo-density matrix formulation to time crystals. By defining time crystals as long-range order in time, we analyse continuous and discrete time translation symmetry as well as discuss the existence of time crystals from an algebraic point of view. Finally, we summarise our work and provide the outlook for future directions.

==> chapter/abbreviations.tex <==
% First parameter can be changed eg to "Glossary" or something.
% Second parameter is the max length of bold terms.
\begin{mclistof}{List of Abbreviations}{3.2cm}

\item[1-D, 2-D] One- or two-dimensional, referring in this thesis to spatial dimensions in an image.

\item[Otter] One of the finest of water mammals.

\item[Hedgehog] Quite a nice prickly friend.

\end{mclistof} 


==> chapter/ch6-otoc.tex <==
%\begin{savequote}[8cm]
%Alles Gescheite ist schon gedacht worden.\\
%Man muss nur versuchen, es noch einmal zu denken.
%
%All intelligent thoughts have already been thought;\\
%what is necessary is only to try to think them again.
%  \qauthor{--- Johann Wolfgang von Goethe \cite{von_goethe_wilhelm_1829}}
%\end{savequote}

\chapter{\label{ch:6-otoc}Application: out-of-time-order correlation functions (OTOCs) and black holes}

\minitoc

\section{Brief introduction for out-of-time-order correlation functions (OTOCs)}
%In this section, we introduce out-of-time-order correlation functions (OTOCs) and briefly discuss why they are interesting. 

%\subsection{Definition for OTOC}

Out-of-time-ordered correlation functions (OTOCs) are usually defined as 
\begin{equation}
\langle V(0)W(t)V^{\dag}(0)W^{\dag}(t) \rangle \equiv \frac{1}{d} \Tr[V(0)W(t)V^{\dag}(0)W^{\dag}(t)] \ \ \rho = \frac{\mathbbm{1}}{d}.
\end{equation}
Note that it is usually defined for the thermal state $\rho = \frac{\mathbbm{1}}{d}$.
Consider a correlated qubit chain. Measure $V$ at the first qubit and $W$ at the last qubit. Since the chain is correlated in the beginning, we have OTOC as $1$. As time evolves and the operator growth, OTOC will approximate to $0$ at the late time. 


%\subsection{Properties of OTOC}

\section{Relation with pseudo-density matrix formalism}
In this section we make a connection between OTOCs and pseudo-density matrix formalism. If we consider a qubit evolving in time and backward, we can get a tripartite pseudo-density matrix. 
In particular, if we consider measuring $A$ at $t_1$, $B$ at $t_2$ and $A$ again at $t_3$ and assume the evolution forwards is described by $U$ and backward $U^{\dag}$. 
Then the probability is given by 
\begin{equation}
\Tr[A U^{\dag} B U A \rho A^{\dag} U^{\dag} B^{\dag} U A^{\dag}] = \Tr[A B(t) A \rho A^{\dag} B^{\dag}(t) A^{\dag}] 
\end{equation}
If we assume that $AA^{\dag} = A$, $\rho = \frac{\mathbbm{1}}{d}$, it will reduce to OTOC. 

\section{Black hole final state proposal}
\subsection{Review on black hole information paradox}

\subsection{Final state projection proposal}

\subsection{OTOC analysis for final state proposal}

%\section{Introduction}
%
%This document introduction won't serve as a complete primer on \LaTeX.  There are plenty of those online, and googling your questions will often get you answers, especially from \url{http://tex.stackexchange.com}.
%
%Instead, let's talk a little about a few of the features and packages lumped into this template situation.  The \verb|savequote| environment at the beginning of chapters can add some wittiness to your thesis.  If you don't like the quotes, just remove that block.
%
%For when it comes time to do corrections, there are two useful commands here.  First, the \verb|mccorrect| command allows you to highlight a short correction \mccorrect{like this one}.  When the thesis is typeset normally, the correction will just appear as part of the text.  However, when you declare \verb|\correctionstrue| in the main \verb|Oxford_Thesis.tex| file, that correction will be highlighted in blue.  That might be useful for submitting a post-viva, corrected copy to your examiners so they can quickly verify you've completed the task.
%
%\begin{mccorrection}
%For larger chunks, like this paragraph or indeed entire figures, you can use the \verb|mccorrection| environment.  This environment highlights paragraph-sized and larger blocks with the same blue colour.
%\end{mccorrection}
%
%Read through the \verb|Oxford_Thesis.tex| file to see the various options for one- and two-sided printing, including or excluding the separate abstract page, and turning corrections and draft footer on or off, and the separate option to centre your text on the page (for PDF submission) or offset it (for binding).  There is also a separate option for master's degree submissions, which changes identifying information to candidate number and includes a word count.  (Unfortunately, \LaTeX has a hard time doing word counts automatically, so you'll have to enter the count manually if you require this.)
%
%\section{Cardiac Imaging}\label{app:imaging}
%
%Within months of Röntgen's discovery of the X-ray in \mccorrect{1895}\cite{gagliardi_rontgen_1996}, cardiac pathology was being investigated via non-invasive imaging \cite{gagliardi_cardiac_1996}.  Over the intervening years, cardiac imaging modalities and techniques have advanced significantly.  Clinically, cardiac imaging is used for two broad purposes: diagnosis of pathophysiology and guidance of interventional procedures.  These applications impose different requirements on imaging equipment, image acquisition time, computational complexity, spatial and temporal resolution, and tissue discrimination.  The common diagnostic and interventional cardiac imaging techniques in current clinical practice are reviewed below.  An accessible introduction to the physics of medical imaging can be found in Webb's \textit{Introduction to Biomedical Imaging} \cite{webb_introduction_2002}.  A comprehensive overview of the use of imaging in clinical cardiology is presented in Leeson's \textit{Cardiovascular Imaging} \cite{leeson_cardiovascular_2011}.
%
%\subsection{Diagnostic Imaging}
%\label{sub:diagnostic}
%
%Beyond the chest X-ray (`plain film'), the key non-invasive imaging modalities in diagnostic cardiology are echocardiography, magnetic resonance imaging, and X-ray computed tomography, which are reviewed below.  Nuclear medicine, including positron emission tomography (PET) and single-photon emission computed tomography (SPECT), are not discussed here, as they do not play a role in the chapters to follow.
%
%\subsubsection{Echocardiography}
%
%\begin{figure}
%\centering\includegraphics[width=0.7\textwidth]{figures/sample/Gray498.png} 
%\caption[Four-chamber illustration of the human heart.]{Four-chamber illustration of the human heart.  Clockwise from upper-left: right atrium, left atrium, left ventricle, right ventricle.}
%\label{fig:fourchamber}\end{figure}
%
%The use of acoustic waves for medical diagnosis, inspired by naval sonar, was initially developed in the 1940s \cite{gagliardi_ultrasonography_1996}.  By 1954, the first clinically useful cardiac ultrasound -- examining motion of the mitral valve in stenosis -- was reported \cite{edler_ultrasonic_1957}.  These early scans were one-dimensional images (`A-mode'), sometimes repeated to generate a time axis (`M-mode').   The sector-scanning probe was developed in the 1970s \cite{bom_ultrasonic_1971,griffith_sector_1974}, leading to the `B-mode' that a modern cardiologist would recognise as an echocardiogram.

